EMMA-X: An EM-like Multilingual Pre-training Algorithm for Cross-lingual Representation Learning

Expressing universal semantics common to all languages is helpful in understanding the meanings of complex and culture-specific sentences. The research theme underlying this scenario focuses on learning universal representations across languages with the usage of massive parallel corpora. However, due to the sparsity and scarcity of parallel data, there is still a big challenge in learning authentic ``universals'' for any two languages. In this paper, we propose EMMA-X: an EM-like Multilingual pre-training Algorithm, to learn (X)Cross-lingual universals with the aid of excessive multilingual non-parallel data. EMMA-X unifies the cross-lingual representation learning task and an extra semantic relation prediction task within an EM framework. Both the extra semantic classifier and the cross-lingual sentence encoder approximate the semantic relation of two sentences, and supervise each other until convergence. To evaluate EMMA-X, we conduct experiments on XRETE, a newly introduced benchmark containing 12 widely studied cross-lingual tasks that fully depend on sentence-level representations. Results reveal that EMMA-X achieves state-of-the-art performance. Further geometric analysis of the built representation space with three requirements demonstrates the superiority of EMMA-X over advanced models.

==> tex/experiments_original.tex <==

We conduct experiments from two perspectives: (1) Evaluation on the \textbf{\textsc{xrete}} benchmark, verifying the transfer ability of \textsc{Emma}-X on various cross-lingual downstream tasks. (2) Geometry analysis, directly evaluating the satisfaction of the built representation space on three pre-defined requirements (i.e., invariance, {canonical form} and {isotropy}). 

\subsection{Setup}

\noindent\textbf{Corpus} We collect parallel corpora from CCAligned \citep{el-kishky-etal-2020-ccaligned}, CCMatrix \citep{schwenk-etal-2021-ccmatrix}, WMT \citep{akhbardeh-etal-2021-findings}, and MultiUN \citep{ziemski-etal-2016-united}, involving 94 languages with more than 4.8 billion sentence pairs. In addition, we add CC-100 \citep{conneau-etal-2020-unsupervised}, which is a large-scale monolingual corpus that covers 94 languages. The statistics of all data are provided in \textbf{Appendix \ref{appendix:pretraining-data}}.

\noindent\textbf{Model} The cross-lingual encoder starts from the well-trained \textsc{Xlm-r} large model \citep{conneau-etal-2020-unsupervised}, with 24 layers of Transformer \citep{Vaswani2017Attention} encoder, 1024 hidden states and 16 attention heads. The GMM classifier is implemented as a mixture of four Gaussian forms, each of which consists of a prior $\pi \in \mathbb{R}^1$, a mean $\mu \in \mathbb{R}^{1024}$ and a variance $\sigma \in \mathbb{R}^{1024}$, both are trainable variables.  Hyperparameters are shown in \textbf{Appendix \ref{appendix:pretraining-data}}.

\subsection{\textsc{xrete} Evaluation}
\textbf{\textsc{xrete}} includes 12 cross-lingual tasks that fall into 4 different categories depending fully on cross-lingual sentence-level representations, with 7 tasks from XTREME(-R) and 5 novel and challenging tasks containing different long-tail languages. Refer to \textbf{Appendix \ref{app:benchmark_info}} and \textbf{\ref{app:baseline_info}} for details of \textsc{xrete} and baselines. Empirical results are shown in Table~\ref{tbl:main-results}.

\begin{table*}[t]
\begin{center}
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Inference}} & \multicolumn{2}{c}{\textbf{Similarity}} & \multicolumn{4}{c}{\textbf{Retrieval}} 
& \multicolumn{4}{c}{\textbf{Classification}}
\\
& XNLI & ANLI & STS & QE & LAReQA & Mewsli-X & BUCC & Tatoeba & XCOPA & EURLEX & ARC & PAWS-X\\
\cmidrule{1-13}
Metrics & Acc. ($\color{green}{\uparrow}$) & Acc. ($\color{green}{\uparrow}$) & Spearman ($\color{green}{\uparrow}$) & Pearson ($\color{green}{\uparrow}$) & mAP@20 ($\color{green}{\uparrow}$) & mAP@20 ($\color{green}{\uparrow}$) & F1 ($\color{green}{\uparrow}$) & Acc. ($\color{green}{\uparrow}$) & Acc. ($\color{green}{\uparrow}$) & Acc. ($\color{green}{\uparrow}$) & MAE ($\color{red}{\downarrow}$) & Acc. ($\color{green}{\uparrow}$)\\
\midrule
\textsc{mBert}$^*$ & 75.1$^a$ & - & 55.8$^s$ & - & 21.6$^d$ & 38.6$^d$ & 56.7$^a$ & 39.0$^a$ & 56.1$^d$ & 67.4$^s$ & 48.2$^s$ & 81.9$^a$ \\
\textsc{Xlm}$^*$ & 77.8$^b$ & - & - & - & - & - & 56.8$^a$ & 32.6$^a$ & - & - & - & 80.9$^a$ \\
\textsc{Xlm-r}$^*$ & 83.6$^b$ & 49.12$^s$ & 61.5$^s$ & 0.587$^s$ & 40.7$^d$ & 45.7$^d$ & 66.0$^a$ & 57.7$^a$ & 69.2$^d$ & 66.6$^s$ & - & 88.9$^a$ \\
\textsc{Hictl}$^*$ & 84.7$^c$ & - & - & - & - & - & 77.6$^c$ & 69.1$^c$ & - & - & - & 92.8$^c$ \\
\textsc{LASER}$^*$ & 84.7$^c$ & - & - & - & - & - & 77.6$^c$ & 69.1$^c$ & - & - & - & 92.8$^c$ \\
\textsc{ChatGPT} & 60.9 & 41.7 & - & - & - & - & - & - & 74.2 & - & - & 64.2 \\
\midrule
\multicolumn{13}{l}{\emph{Ours re-implementation, directly evaluate on tasks without fine-tuning (zero-shot)}} \\
\midrule
\textsc{SBERT} & - & - & \textbf{84.0} & 0.393 & \textbf{31.8} & - & 88.5 & 68.6 & - & - & - & - \\
\textsc{LaBSE} & - & - & 74.4 & 0.316 & 12.8 & - & \textbf{93.2} & \textbf{83.6} & - & - & - & - \\
\textsc{XLM-R} & - & - & 25.0 & 0.104 & 16.1 & 11.7 & 67.9 & 59.1 & - & - & - & - \\
\textsc{InfoXLM} & - & - & 55.2 & 0.494 & 16.9 & 23.9 & 77.4 & 66.2 & - & - & - & - \\
\textbf{\textsc{Emma-X}} & - & - & 62.9 & \textbf{0.547} & 19.4 & \textbf{29.4} & 81.9 & 72.9 & - & - & - & - \\
\midrule
\multicolumn{13}{l}{\emph{Ours re-implementation, fine-tune cross-lingual model on all training sets (Translate-train-all)}} \\
\midrule
\textsc{Xlm-r}$^\ddag$ & 82.8 & 48.48 & 65.9 & 0.632 & 40.3 & 48.6 & - & - & 71.2 & 66.9 & 44.9 & 90.1 \\
\textsc{InfoXLM}$^\ddag$ & 84.2 & 49.10 & 82.2 & 0.641 & 44.9 & 57.1 & - & - & 74.6 & 67.7 & 36.2 & 93.0 \\
% \textsc{Hictl}$^\ddag$ & 85.1 & 49.02 & 81.6 & 0.649 & 46.1 & 54.8 & 77.6 & 65.8 & 74.8 & 68.3 & 38.2 & 92.8 \\
\textsc{Hictl}$^\ddag$ & 85.1 & 49.02 & 81.6 & 0.649 & 46.1 & 54.8 & - & - & 74.8 & 68.3 & 38.2 & 92.8 \\
\textbf{\textsc{Emma-X}} & \bf 88.1 & \bf 50.21 & \bf 87.3 & \bf 0.672 & \bf 50.6 & \bf 59.6 & - & - & \bf 78.2 & \bf 71.4 & \bf 32.7 & \bf 94.2 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results on the \textsc{xrete} benchmark. $^*$ denotes the results from previous literature, $^a$\citet{pmlr-v119-hu20b} $^b$\citet{conneau-etal-2020-unsupervised} $^c$\citet{wei2021on} $^d$\citet{ruder-etal-2021-xtreme}. $^s$ denotes the results from the original paper of the specific task. $^\ddag$ denotes results from our re-trained models with the same model size and training corpora as \textsc{Emma}-X for fairer comparisons. We also provide results on several tasks that are most dependent on universal representations with the zero-shot cross-lingual transfer setting (\textbf{Appendix E}). Refer to \textbf{Appendix F} for greater details on each task and language, which demonstrates that \textsc{Emma-X} performs even better on low-resource languages.}\label{tbl:main-results}
\end{table*}

\begin{table*}[t]
\begin{center}
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccccccccc}
\toprule
\textbf{Model} & \textbf{af} & \textbf{ar} & \textbf{bg} & \textbf{bn} & \textbf{de} & \textbf{el} & \textbf{es} & \textbf{et} & \textbf{eu} & \textbf{fa} & \textbf{fi} & \textbf{fr} & \textbf{he} & \textbf{hi} & \textbf{hu} & \textbf{id} & \textbf{it} & \textbf{ja} \\ 
\midrule
\textsc{Xlm-r} & 59.7 & 50.5 & 72.2 & 45.4 & 89.5 & 61.3 & 77.6 & 51.7 & 38.6 & 71.7 & 72.8 & 76.9 & 66.3 & 73.1 & 65.1 & 77.5 & 68.5 & 63.1 \\
\textsc{InfoXLM} & 63.0 & 50.9 & 76.8 & 47.0 & \textbf{94.6} & 68.8 & 80.9 & 59.3 & 41.5 & 77.3 & 78.2 & 80.3 & 70.2 & 77.9 & 72.1 & 81.3 & 73.7 & 66.2 \\
%\textsc{Emma}-X (Parallel Only) & 66.2 & 54.3 & 79.6 & 49.4 & \textbf{92.9} & 70.5 & 84.9 & 62.6 & 44.5 & 77.9 & 82.1 & 81.4 & 74.4 & 82.6 & 77.1 & \textbf{86.7} & 77.1 & 69.4 \\
\textbf{\textsc{Emma}-X} & \textbf{68.9} & \underline{\textbf{60.2}} & \textbf{83.4} & \underline{\textbf{62.1}} & 92.6 & \textbf{73.0} & \textbf{85.7} & \underline{\textbf{67.3}} & \underline{\textbf{56.4}} & \textbf{78.0} & \underline{\textbf{84.1}} & \textbf{84.1} & {\textbf{76.3}} & {\textbf{83.5}} & \underline{\textbf{81.0}} & \textbf{85.4} & \underline{\textbf{83.6}} & \textbf{73.3} \\ \midrule
 & \textbf{jv} & \textbf{ka} & \textbf{kk} & \textbf{ko} & \textbf{ml} & \textbf{mr} & \textbf{nl} & \textbf{pt} & \textbf{ru} & \textbf{sw} & \textbf{ta} & \textbf{te} & \textbf{th} & \textbf{tl} & \textbf{tr} & \textbf{ur} & \textbf{vi} & \textbf{zh} \\ 
\midrule
\textsc{Xlm-r} & 15.8 & 53.5 & 51.2 & 63.1 & 66.2 & 59.0 & 81.0 & 84.4 & 76.9 & 19.8 & 28.3 & 37.8 & 28.9 & 36.7 & 68.9 & 26.6 & 77.9 & 69.8 \\
\textsc{InfoXLM} & 19.6 & 57.3 & 54.6 & 68.0 & 71.8 & 62.0 & 88.1 & 88.9 & 77.7 & 26.1 & 32.9 & 39.5 & 32.9 & 43.2 & 71.2 & 27.8 & 79.9 & 74.7 \\
%\textsc{Emma}-X (Parallel Only) & 17.9 & 61.8 & 57.1 & 70.6 & \textbf{73.9} & 65.3 & \textbf{91.4} & 92.1 & 80.8 & 27.5 & 37.4 & 42.3 & 36.7 & 48.1 & 74.6 & 32.3 & \textbf{82.1} & 78.8 \\
\textbf{\textsc{Emma}-X} & \textbf{24.7} & \underline{\textbf{66.2}} & \underline{\textbf{65.0}} & \textbf{73.4} & \textbf{73.7} & \textbf{66.8} & \textbf{89.6} & \textbf{92.7} & \textbf{83.6} & \underline{\textbf{51.2}} & \underline{\textbf{47.8}} & \underline{\textbf{50.4}} & \underline{\textbf{51.9}} & \underline{\textbf{60.7}} & \textbf{76.5} & \underline{\textbf{49.4}} & \textbf{80.3} & \underline{\textbf{84.6}} \\ 
\bottomrule
\end{tabular}}
\end{center}
\caption{Evaluation results on 36 languages on Tatoeba~\citep{artetxe-schwenk-2019-massively}. Best results are marked with bold font. We highlight greatly improved results with underlines.}\label{tbl:tatoeba-38-eval}
\end{table*}

\begin{table*}[ht]
\begin{center}
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Top-20 Langs.}} & \multicolumn{3}{c|}{\textbf{69 Langs. Commonly Covered by All Models}} & \multicolumn{3}{c}{\textbf{All 204 Langs.}} \\
% \cmidrule{2-4,5-7,8-10}
& Invariance & Canonical Form & Isotropy & Invariance & Canonical Form & Isotropy & Invariance & Canonical Form & Isotropy\\
\midrule
Metrics & KL-D. ($\color{red}{\downarrow}$) & CH-I. ($\color{green}{\uparrow}$) & PR ($\color{green}{\uparrow}$) & KL-D. ($\color{red}{\downarrow}$) & CH-I. ($\color{green}{\uparrow}$) & PR ($\color{green}{\uparrow}$) & KL-D. ($\color{red}{\downarrow}$) & CH-I. ($\color{green}{\uparrow}$) & PR ($\color{green}{\uparrow}$)\\
\midrule
\textsc{Xlm-r} (cls) & 0.3570 & 16.31 & 0.3681 & 0.7356 & 30.19 & 0.3681 & 1.6501 & 20.80 & 0.3683\\
\textsc{Xlm-r} (mean) & 0.6036 & 9.95 & 0.3687 & 1.5017 & 16.07 & 0.3689 & 2.0465 & 15.46 & 0.3694\\
% \textsc{Xlm-r} (mean) & 25.0 & 0.104 & 3.4 & 11.7\\
\textsc{InfoXLM} (cls) & 0.1780 & 27.63 & \bf 0.4289 & 0.4491 & 38.82 & 0.4478 & 1.4747 & 31.51 & 0.4665\\
%\textsc{InfoXLM} (mean) & 0.6359 & 9.95 & 0.4009 & 1.3143 & 16.47 & 0.4065 & 2.3110 & 16.80 & 0.4120\\
\midrule
\textsc{Emma-X} (cls) & \bf 0.1594 & \bf 29.83 &  0.4176 & \bf 0.3603 & \bf 43.52 & \bf 0.5318 & \bf 1.1904 & \bf 48.70 & \bf 0.5918\\
\bottomrule
\end{tabular}}
\end{center}
\caption{Comparison with existing methods on geometric analysis. We directly evaluate the sentence representations on FLORES dataset~\citep{costa2022no} without fine-tuning. ``Top-20 Langs.'' means the top 20 languages covered by CC-100~\citep{conneau-etal-2020-unsupervised} with the richest resources. ``cls'' and ``mean'' represent two different pooling strategies to obtain sentence representations.}\label{tbl:geo-analysis}
\end{table*}

%\subsubsection{Results on XRETE}
%\label{main-results}

\noindent\textbf{Cross-lingual NLI} \textsc{Emma}-X achieves 88.1\% on XNLI~\citep{conneau-etal-2018-xnli} and 50.21\% on ANLI~\citep{ebrahimi-etal-2022-americasnli}, outperforming all baseline models (\textsc{Xlm-r}~\citep{conneau-etal-2020-unsupervised}, \textsc{Hictl} \citep{wei2021on} and \textsc{InfoXLM} \citep{chi-etal-2021-infoxlm}) with up to 5.3\% improvements. This reveals that \textsc{Emma}-X obtains better cross-lingual transferability from universal representations.

\noindent\textbf{Cross-lingual Semantic Similarity} \textsc{Emma}-X gains the highest results among all baselines on both WMT21-QE-Task1~\citep{specia-etal-2021-findings} and Multi-STS~\citep{reimers-gurevych-2020-making} tasks. On the Multi-STS task, \textsc{Emma}-X achieves an 87.3 correlation score, outperforming several strong baselines by 5.1$\sim$22.5, and \textbf{even achieves comparable performance between the cross-lingual and the monolingual settings} (see \textbf{Appendix F} for language-specific results). Furthermore, \textsc{Emma}-X obtains a 0.672 Pearson score on QE task, which is comparable to the winner on the leaderboard\footnote{\url{https://www.statmt.org/wmt21/quality-estimation-task_results.html}} without any specific finetuning techniques.

\noindent\textbf{Cross-lingual Sentence Retrieval} Following the standard setting, we report the mAP@20 metric on both LAReQA~\citep{roy-etal-2020-lareqa} and Mewsli-X~\citep{ruder-etal-2021-xtreme} tasks, but F1 and accuracy on BUCC~\citep{zweigenbaum-etal-2017-overview} and Tatoeba~\citep{artetxe-schwenk-2019-massively}, respectively. As illustrated in Table~\ref{tbl:main-results}, \textsc{Emma}-X consistently outperforms previous strong baselines among all 4 tasks, and demonstrates 10\%$\sim$16\% improvements over these baselines.

\noindent\textbf{Cross-lingual sentence classification} We report the MAE score on the ARC task , while top-1 accuracy scores on others. \textsc{Emma}-X obtains an 81.3\% top-1 accuracy averaged on XCOPA~\citep{ponti-etal-2020-xcopa}, EURLEX~\citep{chalkidis-etal-2021-multieurlex} and PAWS-X~\citep{yang-etal-2019-paws} tasks, outperforming \textsc{Xlm-r}, \textsc{InfoXLM} and \textsc{Hictl} (demonstrating 76.0\%, 78.4\% and 78.6\% top-1 accuracies) by 5.3\%, 2.9\% and 2.7\% improvements, respectively. On ARC~\citep{keung-etal-2020-multilingual} task, \textsc{Emma}-X shows the lowest error rates among all models.


\noindent\textbf{Representation Collapse of Long-tail Languages}
Existing models rely heavily on parallel corpora, which are sparsely distributed across languages, leading to the representations learnt for massive long-tail languages collapsed. To study this, we report the results on Tatoeba~\citep{artetxe-schwenk-2019-massively} which involves several long-tail languages in Table \ref{tbl:tatoeba-38-eval}. We can observe that \textsc{Emma}-X significantly outperforms \textsc{Xlm-r} and \textsc{InfoXLM} by 12.2\% and 8.1\% on average among all languages. On multiple long-tail languages (the underlined part), \textsc{Emma}-X substantially improves top-1 accuracy by 10\%$\sim$32\%. This confirms that \textsc{Emma}-X has a great potential on mitigating the representation discrepancy between few head and massive long-tail languages.

\subsection{Geometry Analysis}
To interpret the advantages of \textsc{Emma-X}, we evaluate the geometric characteristics of \textsc{Emma}-X on FLORES-200 dataset \citep{costa2022no} , which contains manual translations in 204 languages (total 3001 sentences). The criteria of three requirements are listed as follows.

\noindent\textbf{Invariance Measurement} implies whether the semantic distributions of all languages are similar~\citep{abend-rappoport-2017-state}. We adopt a Gaussian form ${\scriptstyle \mathcal{N}_l(\mu_l,\sigma_l^2)}$ where ${\scriptstyle \mu_l=\frac{\sum_{\mathbf{x} \in l}\gamma^{(\mathbf{x})}}{3001}}$ and ${\scriptstyle \sigma_l^2= \sum_{\mathbf{x} \in l} (\gamma^{(\mathbf{x})} -\mu_l)(\gamma^{(\mathbf{x})} -\mu_l)^T}$, to approximate the semantic distribution of each language $l$. Further, we compute the mean averaged KL-divergence (KL-D. for short)~\citep{10.1214/aoms/1177729694} among all language pairs as the overall Invariance score $\boldsymbol{\scriptstyle \mathcal{I}_v}$ with $L$ as the total number of languages: 
\begin{equation}
\scriptsize
    \mathcal{I}_v = \frac{1}{L \times (L-1)} \sum_{l_1 \neq l_2} \frac{\mathbf{KL}(\mathcal{N}_{l_1} || \mathcal{N}_{l_2}) + \mathbf{KL}(\mathcal{N}_{l_2} || \mathcal{N}_{l_1})}{2},
\end{equation}

\noindent\textbf{Canonical Form Measurement} Previous works \citep{10.1162/089120100750105975,irwin2009methodology} have demonstrated that a good multilingual space should distribute sentence representations based on their semantic similarities rather than language families. To measure this in quantity, we focus on Calinski-Harabasz Index (CH-I.) \citep{doi:10.1080/03610927408827101}, which measures how similar an object is to its own cluster compared to other clusters. We group all semantically equivalent sentences in a cluster, which leads to 3001 clusters and each obsesses 204 sentences in 204 different languages. Assuming $c_k$ and $c$ are the centroid of cluster $k$ and the whole dataset ${\scriptstyle \mathcal{S}}$, respectively. The CH-I. $\boldsymbol{\scriptstyle \mathcal{C}_h}$ is defined as:
\begin{equation}
    \scriptsize
    \mathcal{C}_h = \Big[ 204 \times \sum_{k=1}^{K} \Vert c_k - c \Vert ^2 \Big] / \Big[ \sum_{k=1}^{K} \sum_{s \in \mathcal{S}} \Vert s - c_k \Vert ^2 \Big].
\end{equation}
The higher the CH-I. is, the better the semantically equivalent sentences are clustered.

\noindent\textbf{Isotropy Measurement} A high dimensional embedding space often demonstrates poor isotropy, and deteriorates into a low-dimensional manifold that greatly limits the expressive ability of the embedding space. We adopt principal ratio (PR)~\citep{mu2018allbutthetop} to measure isotropy. Let $\boldsymbol{\scriptstyle \mathcal{E}}$ be the sentence representation matrix, $\boldsymbol{\scriptstyle \mathcal{V}}$ be the set of the eigenvectors of $\boldsymbol{\scriptstyle \mathcal{E}}$, the Isotropy $\boldsymbol{\scriptstyle \mathcal{I}_{so}}$ is
\begin{equation}
    \footnotesize
    \mathcal{I}_{so} = {\min_{v \in \mathcal{V}}  \sum_{e \in \mathcal{E} } \exp({v^{\mathsf{T}}e}) } / {\max_{v \in \mathcal{V}}  \sum_{e \in \mathcal{E} } \exp({v^{\mathsf{T}}e}) }.
\end{equation}
The closer $\boldsymbol{\scriptstyle \mathcal{I}_{so}}$ is to $1$, the more isotropic the representation space is. 

\noindent\textbf{Performance}
Results in Table~\ref{tbl:geo-analysis} demonstrate that \textsc{Emma}-X satisfies better than existing models on three measurements. On the top 20 languages, \textsc{Emma}-X improves the performance by 8\% on average of the three measurements over the strongest baseline, despite the fact that all models do well. As the number of languages increases, \textsc{Emma}-X begins to show significant improvements over baselines. Specifically, \textsc{Emma}-X exceeds \textsc{Xlm-r} by over 30\% on average. On Canonical Form measurement, \textsc{Emma}-X even surpasses \textsc{InfoXLM} by over 50\% and \textbf{surprisingly achieves better performance on all 204 languages than on 69 languages}. To intuitively understand the great potential of \textsc{Emma}-X on building a real universal representation space over much more languages, we randomly select 20 languages from FLORES-200 and depict the performance as illustrated in Figure \ref{fig:geometry_analysis}.

\begin{figure*}[t]
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/xlmr_kl_div_2d_crop.pdf}
    \caption{\textsc{Xlm-r} (Invariance)}
    \label{fig:/xlmr_kl_div_2d_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/infoxlm_kl_div_2d_crop.pdf}
    \caption{\textsc{InfoXLM} (Invariance)}
    \label{fig:/infoxlm_kl_div_2d_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/emma_kl_div_2d_crop.pdf}
    \caption{\textsc{Emma}-X (Invariance)}
    \label{fig:/emma_kl_div_2d_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/xlmr_intra_inter_crop.pdf}
    \caption{\textsc{Xlm-r} (Canonical)}
    \label{fig:/xlmr_canonical_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/infoxlm_intra_inter_crop.pdf}
    \caption{\textsc{InfoXLM} (Canonical)}
    \label{fig:/infoxlm_canonical_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.18]{figures/emma_intra_inter_crop.pdf}
    \caption{\textsc{Emma}-X (Canonical)}
    \label{fig:/emma_canonical_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.14]{figures/xlmr_isotropy_crop.pdf}
    \caption{\textsc{Xlm-r} (Isotropy)}
    \label{fig:/xlmr_isotropy_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.14]{figures/infoxlm_isotropy_crop.pdf}
    \caption{\textsc{InfoXLM} (Isotropy)}
    \label{fig:/infoxlm_isotropy_crop}
\end{subfigure}
\begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[scale=0.14]{figures/emma_isotropy_crop.pdf}
    \caption{\textsc{Emma}-X (Isotropy)}
    \label{fig:/emma_isotropy_crop}
\end{subfigure}
\caption{Visualization of representations from \textsc{Emma}-X, \textsc{Xlm-r}~\citep{conneau-etal-2020-unsupervised} and \textsc{InfoXLM}~\citep{chi-etal-2021-infoxlm}. \textsc{Emma}-X demonstrates better performance on cross-lingual identical semantic distribution (c), sentence aggregation based on semantic similarity rather than language (f), and uniform sentence distribution that prevents the representation space from degenerating into a low-dimensional manifold (i).}
\label{fig:geometry_analysis}
\end{figure*}
